Deep Reinforcement Learning with Linear Quadratic Regulator Regions

Practitioners often rely on compute-intensive domain randomization to ensure reinforcement learning policies trained in simulation can robustly transfer to the real world. Due to unmodeled nonlinearities in the real system, however, even such simulated policies can still fail to perform stably enough to acquire experience in real environments. In this paper we propose a novel method that guarantees a stable region of attraction for the output of a policy trained in simulation, even for highly nonlinear systems. Our core technique is to use "bias-shifted" neural networks for constructing the controller and training the network in the simulator. The modified neural networks not only capture the nonlinearities of the system but also provably preserve linearity in a certain region of the state space and thus can be tuned to resemble a linear quadratic regulator that is known to be stable for the real system. We have tested our new method by transferring simulated policies for a swing-up inverted pendulum to real systems and demonstrated its efficacy.

==> old.tex <==

% The \emph{reality gap}, that often renders policies learned in simulation inefficient once transferred onto real systems, remains a critical issue for robotics research and other real-world applications. To  overcome this challenge, existing approaches increase the number of samples with diversified simulated environment parameters (i.e., domain randomization), making the learned policy robust to environment discrepancies at the cost of expensive computation. However, due to unmodeled non-linearities in the real system, such simulated policies can still fail to perform stable enough to continue training in real environments, e.g., a humanoid robot fatally crashing on its first training run. In this paper we propose a novel method that guarantees to output a stable policy from simulation even for highly non-linear systems where inconsistencies between the simulator and real system are present. Our core technique is to use \emp{bias-shifted} neural networks for constructing the controller and training the network in the simulator. The modified neural networks not only capture the non-linearities of the system but also provably preserve linearity in a certain region of the state space and thus resembles a \emph{linear quadratic regulator} that is known to be stable for the real system. We have tested our new method in transferring simulated, learned policies for swing-up inverted pendulums to the real systems and demonstrated its efficacy.
when transferring learned non-linear controllers onto hardware, such that stable training can continue on the hardware to fine tune the weights. In order to do this feedforward neural networks will be used as the function approximators in an actor-critic style deep reinforcement learning algorithm called Twin Delayed Deep Deterministic Policy Gradient (TD3) \cite{fujimoto2018addressing}. Other actor-critic style algorithms will work as long as the function approximators are feedfoward. With a slight restriction on the magnitude of the biases and activation functions with linear parts, \emph{eg} ReLU, a linear region can pass through the network, allowing for a fitting of a linear controller.
% Method Pt. 1--Combining by linear architecture
We propose a method that leverages the stability of known linear feedback controllers when transferring learned non-linear controllers onto hardware, such that stable training can continue on the hardware to fine tune the weights. In order to do this feedforward neural networks will be used as the function approximators in an actor-critic style deep reinforcement learning algorithm called Twin Delayed Deep Deterministic Policy Gradient (TD3) \cite{fujimoto2018addressing}. Other actor-critic style algorithms will work as long as the function approximators are feedfoward. With a slight restriction on the magnitude of the biases and activation functions with linear parts, \emph{eg} ReLU, a linear region can pass through the network, allowing for a fitting of a linear controller.

% Our Approach Pt. 3--Last layer parameter optimization
Once this neural network architecture with a linear region trained to convergence in simulation, the last layer's parameters are modified such that the weighted linear combination of the output of the last layer matches the linear feedback controller known to work on the hardware for some linearized region. By only replacing the last layer parameters, many of the nonlinear feature space will still be preserved in the hidden layers. Retraining the last layer has been used throughout the image processing community for fine tuning for a task \cite{sharif2014cnn} \cite{razavian2016visual} \cite{babenko2014neural} \cite{gong2014multi}. Depending on the task, different layers may be chosen for retraining \cite{yue2015exploiting}.

% Our Verification: Swing-up Pendulum
The running example in simulation and in hardware that we use to verify our approach is the swing-up pendulum. One end of the pendulum is connected to a mass and the other to an actuator. The goal of this environment is to swing up and balance the mass vertically. The actuator is torque limited such that there isn't enough torque to directly drive the pendulum to its upright position. It has to pump up to build enough momentum first to reach its goal. There exists a region that can be linearized where the LQR controller works optimally. Outside of that region though the LQR fails.

% Our Verification: Methodology
The goal of the experimentation is to verify a stable training routine from simulation to hardware. This means that once the model is optimized to produce, in our case, the LQR optimal controller, we can safely begin training in that linear region to help tune the last layer parameters to an optimal solution. As we collect more data we can begin to train in non-linear regions without experiencing instability. In the pendulum's case instability would be the pendulum possibly whipping the top without stopping at the top to balance.

As far as we know, we haven't come across an approach similar to ours. \textbf{TALK ABOUT OTHER APPROACHES OF UTILISING LQR LIKE LIN YANG'S PAPER OR OTHERS AND HOW OURS IS DIFFERENT.}

% Contributions
This paper aims to make the following contributions:
\begin{itemize}
\item Design neural network architectures that have linear or quadratic regions.
\item Develop an optimization problem such that within the linear region for the actor network it outputs the LQR controller and within the quadratic region of the critic network it outputs the LQR optimal cost.
\item Introduce a new method for stably transferring learned policies to real world systems.
\item Verify and analyze this technique on a simple swing-up pendulum environment in simulation and hardware.
\end{itemize}

\lin{Ref. Outline: 1) Our framework: how the new algorithm is going to work? what are the critical steps and components (e.g. pseudocode and the introduction of the new NN architecture). 2) New NN (subsec1, the structure. sub2, the training method. sub3, the expressiveness). 3) How New NN helps? It converts TD3 policy to LQR policy. It converts TD3 value to LQR cost. 4) Experiments}

As far as we know we have not come across any publications involving the creation of a linear region in a feedforward network and trying to shape it. There have been publications on the expressivity of deep feedforward networks where the number of possible linear regions were used as a metric \cite{montufar2014number} \cite{pascanu2013number}.

Other approaches take advantage of LQR or its structure. \cite{du2019continuous} builds a decoder that maps to a linear representation where LQR can be used in new environments. \cite{marco2017design} uses a Gaussian process with kernels that take advantage of the LQR structure. \cite{bradtke1993reinforcement} uses the LQR structure for $Q$-value functions.

Recently, there have been much interest in domain randomization to transfer learned policies to hardware. \cite{akkaya2019solving} uses domain randomization on environments including color to get a robotic hand to solve a Rubik's cube. Several other papers \cite{peng2018sim} randomizes the dynamics in the simulation. \cite{tan2018sim} uses system identification to build a model of their actuators in the simulator in addition to domain randomization. \cite{chebotar2019closing} uses domain randomization but uses real rollouts to



Improve simulator
\cite{tan2018sim} uses sys ID to build better model actuator model in simulator w/ randomizing environments
\cite{chebotar2019closing} uses domain randomization with distributions of environments but uses real rollouts to change parameters in enironments
\cite{james2019sim} uses generator for domain randomization of simulation, uses real images and maps back to simulator environment for testing
\cite{golemo2018sim} trains rnn to learn difference between real and sim then us to make sim better
\cite{carlson2019sensor} models difference between sensor/camera real and sim and adjust sim
\cite{hwangbo2019learning} models motor dynamics in addition to ADR

Building in robustness
\cite{turchetta2019robust} adds delay margin and gain margin metrics for robustness in RL policy
\cite{han2019h_} robust and stability bounds finds Lyapunov function as critic and corresponding policy with guarantees
\cite{harrison2020adapt} uses an MPC to stablize around the trajectory in real world

where $x_0$ is the initial state. The LQR solution for the controller and cost yield a closed form expression for a linear controller and a quadratic optimal cost. With a linear region in the feedforward network of the actor, the weights in the last layer can be fit to this linear controller while a similar fit can be performed on a network with an approximated quadratic region of the optimal cost \textbf{ADD SEE APPENDIX HERE? OR TAKE OUT?}.

In the reinforcement learning context, it too has a controller called a policy taken to be $\pi$ and a reward function, which is the negative cost, called the $Q$-value function, not to be confused with the $Q$ weight matrix in the LQR formulation. For our choice of algorithms $\pi$ will often be referred to as the actor and the $Q$-value function the critic. In reinforcement learning state, $x(t)$ is simply denoted as $s$ and control input or action, $u(t)$, is denoted as $a$. For consistency purposes and to draw a better comparison the notation will remain consistent with Sec. \ref{Sec:Linear Quadratic Regulator}. The policy can be defined as:
\begin{equation*}
    \pi(x(t))=u(t)
\end{equation*}
And the $Q$-value function is given by the following:
\begin{equation*}
    Q(x(t), u(t))=\mathbb{E}\bigg[\sum^N_{t'=t}\gamma^t'r_{t'+1}\big|x_0=x(t), u_0=u(t)\bigg]
\end{equation*}

% Absorbing state
One of the main difference that we will see later is that in the reinforcement learning context the reward function may vastly differ from the actual cost function given by Eq. \ref{Eq:lqr_cost_int}. This will not affect the fitting in the region we want to fit except when it comes to an exit reward in a terminating state, $\rho_{exit}$. When reaching an absorbing state such as the goal state, there can be an additional reward added on. This will end up biasing the fitting of the optimal cost.

\section{LQR Optimal Cost}
Fitting the LQR optimal cost is not necessary but may be helpful in situations where training continued on the real system and simulation trained $Q$-values contain overestimation bias or aren't representative of the LQR fitted policy. This again optimization is only over the last layer of the critic's function approximator. 

\subsection{Quadratic Region}
\label{Sec:quadratic_region}
From Eq. \ref{Eq:lqr_optimal_cost} the optimal cost fitting would require a quadratic region to be passed through just as we did in the linear case in Sec. \ref{Sec:linear_regions}. Here though the second to the last layer will be chosen to have a Swish activation function. As in Sec. \ref{Sec:linear_regions} we let all previous activation functions be ReLU with bias restrictions for a linear region. Again ReLU may be replaced with any activation function with a linear part. The last layer of the critic is usually left to be linear, which we will assume to be the case for us as well. As in Sec. \ref{Sec:linear_regions}, for the optimization formulation masking the weights and biases allows us to drop the activation function in the linear region for the previous layers before the Swish activation unit.

The Swish function can be broken up into two parts, a linear function $x$ multiplied by a sigmoid function $\frac{1}{1+e^{-x}}$. Approximating the sigmoid with the Maclaurin series gives us the quadratic term we need:
\begin{equation*}
    \frac{x}{1+e^{-x}}\approx\frac{1}{4}x^2+\frac{1}{2}x
\end{equation*}
To further simplify the formulation of the optimization problem we introduce new notation:
\begin{equation*}
\widetilde{W}=\begin{bmatrix}\hat{W}&\hat{b}\end{bmatrix},
\;\hat{x}=\begin{bmatrix}x\\u\end{bmatrix},
\;\widetilde{x}=\begin{bmatrix}\hat{x}\\1\end{bmatrix}
\end{equation*}

% Critic architecture and forward propagation
The architecture of the critic's function approximator will be composed of layers $1$ to $n-2$ activation functions with a linear region, allowing for a similar simplification as in Eq. \ref{Eq:ff_linear}. The $n-1$ layer will be composed of the Swish activation function or any activation function where a quadratic approximation can be made. The last layer $n$ is taken to be linear by convention. This allows us to write the approximation for the forward propagation of the critic's network in a condensed form, where $\odot$ stands for the Hadamard product: 
\begin{equation}
y=W_o\bigg(\frac{1}{4}(\hat{W}\hat{x}+\hat{b})\odot(\hat{W}\hat{x}+\hat{b})+\frac{1}{2}(\hat{W}\hat{x}+\hat{b})\bigg)+b_o
\label{Eq:ff_quad1}
\end{equation}
$W_o$ and $b_o$ are the last layer weights and biases that will be optimized over in the next section.

\subsection{Optimization Formulation}
Eq. \ref{Eq:ff_quad1} has a problem that needs to be resolved for the optimization to work, two variables cannot be multiplied together, in this case $W_o$ and $\hat{x}$. This is no longer an efficiently solvable fit. The workaround proposed here is to get rid of the dependence on $\hat{x}$. By getting the quadratic form of $\hat{x}$ in the same form as Eq. \ref{Eq:lqr_optimal_cost}, the optimization problem no longer depends on $\hat{x}$. Throughout the simplification keep in mind that the resulting output $y$ is a scalar.
\begin{equation*}
\begin{split}
y&=\frac{1}{4}W_{o}\bigg((\widetilde{W}\widetilde{x})\odot
(\widetilde{W}\widetilde{x})\bigg)+\frac{1}{2}W_{o}\widetilde{W}\widetilde{x}+b_{o}\\
&=\frac{1}{4}W_{o}\bigg((\widetilde{W}\widetilde{x})\odot
(\widetilde{W}\widetilde{x})\bigg)+\frac{1}{2}W_{o}\widetilde{W}\widetilde{x}+b_{o}\\
&=\frac{1}{4}W_{o}diag(\widetilde{W}\widetilde{x})\widetilde{W}\widetilde{x}
+\frac{1}{2}W_{o}\widetilde{W}\widetilde{x}+b_{o}\\
&=\frac{1}{4}\widetilde{x}^T\widetilde{W}^T diag(W_{o})\widetilde{W}\widetilde{x}+\frac{1}{2}W_{o}\widetilde{W}\widetilde{x}+b_{o}
\end{split}
\end{equation*}
Expanding terms and grouping them according to their degree of dependence on $\hat{x}$, we can set them equal to the desired values that we want for the optimization. Keeping in mind that negative cost is reward, the quadratic terms grouped become:
\begin{equation}
\frac{1}{4}\hat{x}^T\hat{W}^Tdiag(W_{o})\hat{W}\hat{x}=-x^TPx
\label{Eq:quad_ff_w}
\end{equation}
The biases, terms that don't depend on $x$, can be collected together and should be equivalent to the exit reward, $\rho_{exit}$:
\begin{equation}
\frac{1}{4}\hat{b}^T diag(W_{o})\hat{b}+\frac{1}{2}W_{o}\hat{b}+b_{o}=\rho_{exit}
\label{Eq:quad_ff_b}
\end{equation}
Collecting the terms that are linearly dependent on $x$, we can constrain it to be zero:
\begin{equation}
\begin{split}
&\frac{1}{4}(\hat{b}^Tdiag(W_{o})\hat{W}\hat{x} + \hat{x}^T\hat{W}^Tdiag(W_{o})\hat{b})+\frac{1}{2}W_{o}\hat{W}\hat{x}\\
&\frac{1}{4}(\hat{b}^Tdiag(W_{o})\hat{W}\hat{x} + \hat{b}^Tdiag(W_{o})\hat{W}\hat{x})+\frac{1}{2}W_{o}\hat{W}\hat{x}\\
&\frac{1}{2}(\hat{b}^Tdiag(W_{o})\hat{W}+W_{o}\hat{W})\hat{x}\\
&\hat{b}^Tdiag(W_{o})\hat{W} + W_{o}\hat{W}=0
\end{split}
\label{Eq:quad_ff_x}
\end{equation}
Eq. \ref{Eq:quad_ff_b} and Eq. \ref{Eq:quad_ff_x} can be immediately turned into constraints quite trivially. Eq. \ref{Eq:quad_ff_w} still poses a problme because $\hat{x} \ne x$. To resolve this we make a transformation to expand Eq. \ref{Eq:lqr_optimal_cost} to a quadratic form that depends on states and actions without using the trivial zero solution. Let's assume that we are trying to find the block matrices $A_o$, $B_o$, $C_o$, and $D_o$ to satisfy the following relationship:
\begin{equation}
\begin{split}
    -x^TPx&=
    \begin{bmatrix}
    x\\
    u
    \end{bmatrix}^T
    \begin{bmatrix}
    A_o&B_o\\
    C_o&D_o
    \end{bmatrix}
    \begin{bmatrix}
    x\\
    u
    \end{bmatrix}\\
    &=x^TA_ox+u^TC_ox+x^TB_ou+u^TD_ou\\
    &=x^TA_ox-x^TK^TC_ox-x^TB_oKx+x^TK^TD_oKx\\
    &=x^T(A_o-K^TC_o-B_oK+K^TD_oK)x
\end{split}
\label{Eq:lqr_expanded_cost}
\end{equation}
Now Eq. \ref{Eq:quad_ff_w} can be transformed into the following relationship where the dependency on $\hat{x}$ can be dropped:
\begin{equation*}
    \frac{1}{4}\hat{x}^T\hat{W}^Tdiag(W_{o})\hat{W}\hat{x}=\hat{x}^T\begin{bmatrix}
A_o&B_o\\
C_o&D_o
\end{bmatrix}\hat{x}
\end{equation*}

The optimization fitting problem for the cost becomes the following:
\begin{equation}
\begin{split}
minimize &\;\lVert W_{o}-W_{d} \rVert+\lVert b_{o}-b_{d} \rVert+\lVert \nu + \sum W_{o, i} \rVert\\
subject\;to &\;P+(A_o-K^TC_o-B_oK+K^TD_oK)=0\\
&\;\frac{1}{4}\hat{W}^Tdiag(W_{o})\hat{W}-\begin{bmatrix}
A_o&B_o\\
C_o&D_o
\end{bmatrix}=0\\
&\;\frac{1}{4}\hat{b}^T diag(W_{o})\hat{b}+\frac{1}{2}W_{o}\hat{b}+b_{o} = \rho_{exit}\\
&\;\hat{b}^Tdiag(W_{o})\hat{W} + W_{o}\hat{W}=0\\
&\begin{bmatrix}
A_o&B_o\\
C_o&D_o
\end{bmatrix} \preceq 0
\end{split} 
\label{Eq:opt_cost_1}
\end{equation}
The reason $\nu$ is added so that you can restrain the convexity outside of the quadratic region. For cases where the LQR optimal controller has a high gain, the quadratic region may drastically decrease because the large action will kick it outside of the linear regions in preceding layers to the Swish activation function. The positive side is that by ensuring that the last layer weights are largely negative, we can ensure a convex output as seen in Fig. \ref{Fig:lqr_cost_fit} since Swish acts like ReLU for large inputs. $\nu$ can be tuned to not allow for overestimation bias or to fit the optimal cost function as appropriately outside of the linear region.

\begin{figure}[ht!]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{figures/lqr_cost_fit.png}}
\caption{\emph{Black}: The LQR optimal cost output given by Eq. \ref{Eq:lqr_optimal_cost} for a simulated pendulum environment. \emph{Teal/Blue}: The output of a feedforward network with bias restrictions $|b_i|>0.2$ for layers with a ReLU activation unit. For this region the fit is quite close to the LQR optimal solution. For a fair comparison $u=-Kx$ was used in the feedforward network. The error is larger than in Fig. \ref{Fig:lqr_u_fit} because an approximation for the Swish activation was made.}
\label{Fig:lqr_cost_fit}
\end{center}
\vskip -0.2in
\end{figure}

Deep reinforcement learning models have achieved a high level of performance on nontrivial continuous control tasks \cite{duan2016benchmarking}, but these feats have largely been contained to simulation. This often is due to the differences between the simulated and real world environment, known as the \emph{reality gap}. Often times the unmodeled nonlinearities that occur in the real system will result in a simulation trained policy to fail. For certain classes of hardware, an unstable policy can result in substantial damage, rendering the system inoperable even before completing a trajectory.


In recent years there has been some success in obtaining more robust policies from simulators.
One of the methods is called domain randomization (DR), which trains the policy on a range of simulation parameters that includes the hardware parameters as a subset.
Researchers have been able to get drones and robotic hands to complete difficult tasks with this technique \cite{tobin2017domain, loquercio2019deep,  akkaya2019solving}.
Unfortunately, such a method usually requires expensive computation, e.g., \cite{akkaya2019solving} used 64 NVIDIA V100 GPUs and 920 worker machines with 32 CPU cores for their Rubik's cube task, and the total amount of training experience in simulation for all their experiments amounted to approximately 13 thousand years. 
Another promising direction that has gained traction is to build better simulated models by capturing the nonlinearities of the actual system through deep learning (e.g. \cite{hwangbo2019learning}).
However, such deep learning models is hard to build and has to be meticulously crafted for a specific system.
Moreover, neither DR nor simulated models using deep learning have guarantees for convergence or behavior.

%applying learned models on to hardware by training the model on a range of simulation parameters. 
%By including the hardware parameters as a subset of this range, the model is trained to be more robust to differences between simulation and the real world. This technique is called domain randomization (DR). Researchers have been able to get drones and robotic hands to complete difficult tasks with this technique \cite{tobin2017domain, loquercio2019deep,  akkaya2019solving}.
%Another promising direction that has gained traction is to build better simulated models by capturing the nonlinearities of the actual system through deep learning. The nonlinear model then is used to drive certain dynamics in simulation during training. \cite{hwangbo2019learning} modeled the nonlinearities in the actuator dynamics in combination with DR to get a quadruped robot to walk.
% What are the disadvantages of the existing approaches?
%Unfortunately,  DR usually requires expensive computation, e.g., \cite{akkaya2019solving} used 64 NVIDIA V100 GPUs and 920 worker machines with 32 CPU cores for their Rubik's cube task, and the total amount of training experience in simulation for all their experiments amounted to approximately 13 thousand years. 
%Even if tasks are less complex than the Rubik's cube, DR still has a high computational barrier to entry to achieve stable models on hardware, especially if there are many environment parameters being considered.
%Modeling the nonlinearities with deep learning models on the other hand is hard to build and has to be meticulously crafted for a specific system. \cite{hwangbo2019learning} still combined their simulated model with DR to get desired performance. 
%Moreover, neither DR nor simulated models using deep learning have guarantees for convergence or behavior. %\lin{does our method has this guarantee?}.

%What is the question we are trying to answer?
%In contrast,  control theory provides easy to construct policies and that with theoretical guarantees for convergence or behavior, but only for simple systems, e.g., linear or approximately linear systems. The ideal model would have nonlinearities learned through simulation training, but contain a guaranteed region of convergence to facilitate reliable real world testing. Thus, the question we seek to address in this paper is as follows:

In recent years there has been some success in obtaining more robust policies from simulators.
One of the methods is called domain randomization (DR), which trains the policy on a range of simulation parameters that includes the hardware parameters as a subset.
Researchers have been able to get drones and robotic hands to complete difficult tasks with this technique \cite{tobin2017domain, loquercio2019deep,  akkaya2019solving}.
Unfortunately, such a method usually requires expensive computation, e.g., \cite{akkaya2019solving} used 64 NVIDIA V100 GPUs and 920 worker machines with 32 CPU cores for their Rubik's cube task, and the total amount of training experience in simulation for all their experiments amounted to approximately 13 thousand years. 
Another promising direction that has gained traction is to build better simulated models by capturing the nonlinearities of the actual system through deep learning (e.g. \cite{hwangbo2019learning}).
However, such deep learning models is hard to build and has to be meticulously crafted for a specific system.
Moreover, neither DR nor simulated models using deep learning have guarantees for convergence or behavior.

%\emph{Can nonlinear features of a learned policy in simulation be preserved while guaranteeing a stable regime for experience collection on hardware?}

In this paper, we seek for the more ideal approach that take advantages from both the control theory and DR worlds:
we would like to have class of policies that can be trained in a simulator efficiently, running robust after transferring to the real-world, and being able to improve after seeing more data.
More specifically, we would like to find a policy class that can capture both the linear region and non-linear region of a system such that the policy can be robustly executed within the linear region of the system, which is stable and perturbation resilient, and can continue to improving while non-linearity starts to kick in.

In this paper we seek for the more ideal approach that take advantages from both the control theory and DR worlds:
we would like to have class of policies that can be trained in a simulator efficiently, running robust after transferring to the real-world, and being able to improve after seeing more data.
More specifically, we would like to find a policy class that can capture both the linear region and non-linear region of a system such that the policy can be robustly executed within the linear region of the system, which is stable and perturbation resilient, and can continue to improving while non-linearity starts to kick in.

Fortunately, for many practical systems, e.g., robots, drones and pendulums, there are
pre-existing \emph{robust} linear controllers, which albeit are not performing well compared to the best trained deep-learning based policies.
These controllers nevertheless inspire us to ask the following question.
\emph{
Can we \emph{embed} the prior-known linear feedback controllers into a neural network architecture such that 
the resulting policy can be as rich as the standard neural network and as stable as a linear controller?
%prior-known linear feedback controllers in deep reinforcement learning
}
In this paper, we answer this question affirmatively by proposing a novel neural network structure called the  ``bias-shifted'' neural network to contruct the policy.

The core construction idea comes from the following observation: The nonlinearity of a standard feedforward network comes from its activation functions, which usually can be decomposed into linear parts. For instance, ReLU, defined as $\max(x, 0)$, has two linear parts $(\infty, 0)$ and $[0, \infty)$. We leverage this observation by adding a ``bias-shift'' property in the network such that the response of the neural network to a desired input region can be made approximately linear. 
%if without any activation functions, 
%a feed-forward network is just a linear combination of its inputs.
%Most activation functions generally have at least a portion of their function that is linear or approximately linear, e.g., ReLU and Swish, respectively. 
%Thus, most activation functions can be used in this architecture. By shifting the biases, the activation function can be shifted to a portion that corresponds to the desired input space where linearity is desired. With mild restrictions on the biases' magnitudes and added regularization terms to the loss, linearity can be passed through to the output for a region of the input space.
As we are still using the same set of activation functions and certain number of hidden layers, the non-linearity of the system can be preserved.
To capture the linearity of classic control-theoretical controller, e.g., a policy from a \emph{linear quadratic regulator} (LQR), 
we can either directly adjust the weights of the last layer or add a penalization term as the distance from it to the classic controller when train it in a simulator.
%With such a neural network structure, the non-linearity of the system can be still preserved with the activation functions, and we can fit it to a piror-known linear controller, e.g., a policy from a \emph{linear quadratic regulator} (LQR), by adding a penalty term induced by the linear policy.

%if without any activation functions, 
%a feed-forward network is just a linear combination of its inputs.
%Most activation functions generally have at least a portion of their function that is linear or approximately linear, e.g., ReLU and Swish, respectively. 
%Thus, most activation functions can be used in this architecture. By shifting the biases, the activation function can be shifted to a portion that corresponds to the desired input space where linearity is desired. With mild restrictions on the biases' magnitudes and added regularization terms to the loss, linearity can be passed through to the output for a region of the input space.

To capture the linearity of classic control-theoretical controller, e.g., a policy from a \emph{linear quadratic regulator} (LQR), 
we can either directly adjust the weights of the last layer or add a penalization term as the distance from it to the classic controller when train it in a simulator.
%With such a neural network structure, the non-linearity of the system can be still preserved with the activation functions, and we can fit it to a piror-known linear controller, e.g., a policy from a \emph{linear quadratic regulator} (LQR), by adding a penalty term induced by the linear policy.

%The bias-shifted networks are trained in simulation, and then the last layer parameters are optimized to fit to a linear feedback controller known to be stable on hardware while staying as close as possible to the true parameters. By only modifying the last layer parameters, many of the nonlinear feature space will still be preserved in the hidden layers. Practices like this have been common in the image processing community \cite{sharif2014cnn, razavian2016visual, babenko2014neural, gong2014multi, yue2015exploiting}. Further fine tuning of the last layer can take place on hardware.

% How is the performance?
%The first concern with bias-shifted networks is whether this architecture limits performance. We compared the bias-shifted networks with normal feedforward networks on a suite of continuous control robotics tasks and found increased performance for certain systems and degraded performance in others using an actor-critic style algorithm. We believe this has to do with whether there exists a linear controller for the system near the origin. An additional comparison is done, where the crafted regularization term in the loss is used to embed information about the linear controller to be fit after training. This dramatically increases performance despite the controller being meant for another system.

%Using these bias-shifted networks for a simulated pendulum environment, we verify the veracity of the optimization of the controller. For the linear region an LQR was fitted and modified the policy to give back the LQR in that region. The optimization did change portions of the controller outside of the linear region but remained quite close to the original policy. In some cases for controllers that couldn't complete the task, the optimization adjusted the controller such that the pendulum swung up and completed the task in simulation, although it usually depended on how close the pendulum came to finishing.

%Finally, we transfer our simulated policy to hardware. For the linear region it outputs the LQR that was fitted. As the number of samples we scale up we compare how well our approach does. In the future we will explore procedures of fine tuning the weights of the last layer parameters such that for each trajectory the controller succeeds without experiencing failure in the highly nonlinear regions.

% Contributions
%This paper aims to make the following contributions:
% \begin{itemize}
%\item Introduce bias-shifted neural network architectures.
%\item Develop a procedure to fit a linear stabilizing controller.
%\item Craft regularization terms for bias-shifted networks.
%\item Verify and analyze this on a swing-up pendulum in simulation and hardware.
%\end{itemize}

After training is complete in the simulated environment, the last layer parameters of the network are fed into an optimizer that fits the LQR controller while staying as close as possible to the original weights. Given how many parameters are available in the last layer, adjusting to fit the LQR generally preserves much of the nonlinearities of the policy outside of the linear region. We also introduce a relaxation which checks for stability of the policy output in the linear region and making the LQR constraint into a cost. Sec. \ref{Sec:Optimization Formulation} has more details in regards to this.

Given how many parameters are available in the last layer, adjusting to fit the LQR generally preserves much of the nonlinearities of the policy outside of the linear region. We also introduce a relaxation which checks for stability of the policy output in the linear region and making the LQR constraint into a cost. Sec. \ref{Sec:Optimization Formulation} has more details in regards to this.

% The fitting is depicted in Fig. \ref{Fig:lqr_u_fit} for $|b_i|>0.2$ for all layers. As we can see the fit works quite well. The \emph{black} graph is the LQR optimal control given by Eq. \ref{Eq:lqr_control}, which is linear to the states $x1$ and $x2$. The optimized neural network with linear region shown in \emph{green/teal} fits the LQR close to the origin but as the states get larger the fit doesn't work as well. This is due to the possibly larger weights, $|w_i^Tx| > r$, capable of shrinking the size of the linear region. The linear region is smaller but still achieves the fitting a region.

% Subjecting a stability constraint directly to be inclusive of non-symmetric sets of closed loop stable systems is not convex. The second constraint can also be loosened if the last layer activation function has a large linear region.

% GABES RETUNR MARKER

% To preserve this linear region during training, the biases will be allowed to update but will theoretically be forced by Eq. \ref{Eq:bias_restriction} to at least be larger than the desired linear region $(-m, m)$. In practice desired magnitudes are chosen at the beginning training and left constant throughout. This is in part due to gradient descent updating weights. In Sec. \ref{Sec:Expressiveness and Loss Guidance} we show that this modest restriction isn't detrimental to the performance for continuous control tasks. The effects are only really seen when regularized terms are added as detailed in Sec. \ref{Sec:regularization}.

As seen in Eq. \ref{Eq:ff_linear_exp}, the weights and biases from previous layers can affect the inputs of later layers. The way that we deal with this is by adding additional regularization terms to the loss to penalize updates that would impede upon the linear region. Using the two layer setup from Eq. \ref{Eq:ff_linear_exp}, we can illustrate how to properly formulate the losses. In essence the weights can affect how large the input space is stretched which can effectively shrink the linear region. Following Eq. \ref{Eq:ff_linear_exp} we can show the regularizers on the weights being penalized:
\begin{equation*}
\begin{split}
    \text{(1 Layer) }&\lVert W_1 \rVert\\
    \text{(2 Layers) }&\lVert W_2W_1^m \rVert\\
\end{split}
\end{equation*}
Since there is already a hard constraint on the bias at the first layer given in Algorithm \ref{Alg:TD3training}, the only additional bias regularization we need is:
\begin{equation*}
    \text{(2 Layers) }&-\lVert W_2b_1^m + b_2 \rVert\\
\end{equation*}

we can illustrate how to properly formulate the losses. In essence the weights can affect how large the input space is stretched which can effectively shrink the linear region. Following Eq. \ref{Eq:ff_linear_exp} we can show the regularizers on the weights being penalized:
\begin{equation*}
\begin{split}
    \text{(1 Layer) }&\lVert W_1 \rVert\\
    \text{(2 Layers) }&\lVert W_2W_1^m \rVert\\
\end{split}
\end{equation*}

Since there is already a hard constraint on the bias at the first layer given in Algorithm \ref{Alg:TD3training}, the only additional bias regularization we need is:
\begin{equation*}
    \text{(2 Layers) }&-\lVert W_2b_1^m + b_2 \rVert\\
\end{equation*}

Feedforward networks will serve as the function approximator for the actor and critic throughout, although our technique is not limited to them. Multiple linear layers from this class of networks are simply a combination of weights, $W$, with the input, $x$, and an added bias, $b$, that usually pass through a nonlinear activation function, $\sigma$, to produce output, $y$:
\begin{equation*}
    y=\sigma_n(W_n \ \sigma_{n-1}(... \ \sigma_1(W_1x+b_1) + ...) + b_n)
\end{equation*}
\lin{TODO: add intro of DNN here, introduce bias, weights, etc.}
\lin{Denote $\theta = (W, b)$}

In this section, we introduce our framework for modifying an actor-critic algorithm such that it enjoys the power of an RL algorithm that encodes the nonlinearity of a system but also takes advantages of LQR for the stability.
To begin, we 
%Our approach relies on the fact that we have knowledge 
assume that the system admits a controller (referred as linear controller throughout) that performs stably in a linear or approximately linear region of the hardware, which is usually the case as in our settings, e.g., pendulums. \lin{check}
We propose a 
``bias-shifted'' network 
%(detail description will be presented in the next subsection)
for training the actor network in TD3\footnote{Our framework can also be used to train the critic networks similarly. For presentation simplicity, we only describe the method for training the actor network.}.
%For the sake of presentation, we focus on the actor side in the main text and will discuss how to apply our new network in the critic in the supplementary materials.
After training, the output actor will contain a linear region that matches the existing linear controller.

\paragraph{The Bias-shift Framework}
The ``bias-shift'' framework refers to three phases: initialization, training, and post-training processing. The initialization phase shifts the biases of the actor to be a desired magnitude corresponding to the input affine region.
%of the state space before training begins, constructing a linear region. 
During the training, 
regularization terms are added to the weight matrices to ensure the weights not going too big (which will destroy the linearity provided by the bias).
We also actively shift the biases in the actor network such that the magnitude never goes below the required linear region.
To additionally match the trained actor with the input linear controller, we apply a post-training processing stage.
In this stage, we adjust the last layer of the actor network such that its output matches with the linear controller.
To counter act possible side effects in the post-training fitting, we also add a regularization term to the loss.
%during training.
%regularization terms are also added to the loss during training. This helps counter act the side effects when fitting to a controller post training.

%In the training phase, we 
%can utilize this during training by 
%penalize the distance away from the linear controller analogous to supervised learning in the linear region.
%After training, we tune the last layer parameters to fit the controller better. 
%With this modified training schedule, we are able to encode
%Encoding a 
%the linear controller and at the same time preserve the non-linearity of the original network.
%Tuning this policy on the hardware is guaranteed to be safe since its behavior mimics the linear controller in the linear region.
%After collecting sufficient data, we can additionally tune the parameters of the policy.
%tuned on hardware in this manner can help preserve nonlinear features of the policy while granting a safe region of the state space for real world data collection.
% Critical steps and components: NN and expressiveness
%By enforcing a bias magnitude as shown in

\paragraph{Training}
Our detailed algorithm for training is presented in
Algorithm \ref{Alg:TD3training}.
In the algorithm, we have two critic networks $Q_{\theta_1}$ and $Q_{\theta_2}$.
The update of these networks follow the same way as in the original TD3 algorithm.
We also have an actor network $\pi_{\phi}$, which we will shift its bias actively to avoid the collapsing of the linear region.
The input parameters contain the linear region selector $m$.
In the algorithm, Line~??, we actively restrict all the bias in the actor with magnitude at least $m$.
To keep the weight matrices from going too big, we add an regularization term (Line~???).
%to penalize the distance between the actor and the linear controller.
Note that the critical difference between our algorithm and the original TD3 framework is the bias-shift step (Line~???).




%the activation functions align in such a way that for a portion of the state space a feedforward network outputs a linear combination. Regularization terms on combinations of weights and biases are added to maintain the linear regions during training and nonlinear regions after training when weights are tuned to fit a linear controller. Despite the magnitude constraints and regularizers, Sec. \ref{Sec:Expressiveness and Loss Guidance} demonstrates how our method can greatly outperform the original implementation of TD3 and TD3 with DR on a pendulum.

% Critical steps and components: Optimization
%After training is complete in the simulated environment, the last layer parameters of the network are fed into an optimizer that fits the LQR controller while staying as close as possible to the original weights, as seen in Sec. \ref{Sec:Optimization Formulation}. By only modifying the last layer parameters, many of the nonlinear feature space will still be preserved in the hidden layers. Then when fine tuning the network on hardware the last layer weights receive the direct gradients for update. The image processing community has researched feature space per layer and the utilization of certain layers \cite{sharif2014cnn, razavian2016visual, babenko2014neural, gong2014multi, yue2015exploiting}.

% Pseudocode
\begin{algorithm*}[h]
   \caption{Bias-Shifted TD3 Training}
   \label{Alg:TD3training}
\begin{algorithmic}[1]
    \STATE \textbf{Input:} linear region size: $m\ge 0$; number of iterations $T>0$; number of iterations before updating targets: $d>0$;
    \STATE \textbf{Initialization:}
    \STATE Initialize critic and actor networks: $Q_{\theta_1}$, $Q_{\theta_2}$ and $\pi_\phi$; denote $\phi:= (W, b)$;
    \STATE Initialize target networks: $\theta_1' \leftarrow \theta_1$, $\theta_2' \leftarrow \theta_2$, $\phi'\leftarrow \phi$
    \STATE Initialize replay buffer with random samples $\mathcal{B}$;
    \STATE Initialize biases: sample $b$ by a random number from $[(-c_bm,-m)\cup (m, c_bm)]$  where $c_b>0$ is a parameter;
    %\REPEAT{} 
    %\STATE $b\sim \mathcal{U}(-m, m)\times c_b$,
    %\lin{what is $c_b$?}
    %\UNTIL{$|b|>m$}
    \FOR{$t=1$ {\bfseries to} $T$}
    \STATE Let $a \gets \pi_\phi(s) + \epsilon$, where $\epsilon \sim \mathcal{N}(0, \sigma)$, where $\sigma$ is a parameter to be tuned;
    %\lin{not clear what this means, $\epsilon$-greedy?}
    \STATE At state $s$, execute $a$ to obtain the next state $s'$, and a reward $r$; store ($s, a, r, s'$) in $\mathcal{B}$;
    \STATE Sample $N$ transitions $\{s_l, a_l, r_l, s_l'\}_{l=1}^{N}$ from $\mathcal{B}$
    \STATE
    For each $l\in[N]$: let
    $\tilde a_l \leftarrow \pi_\phi'(s'_l) + \epsilon$, where $\epsilon \sim \mathrm{clip}(\mathcal{N}(0, \sigma), -c, c)$
    and $y_l \leftarrow r_l + \gamma  \min_{i=1,2} Q_{\theta_i'}(s_l', \tilde a_l)$, where $\gamma\in(0,1)$ is a discount factor and $c>0$ is a constant to be tuned;
    \STATE Update critics using least square fitting:\\
     $\qquad\theta_i \gets \underset{\theta_i}{\text{argmin}}\: N^{-1}\sum_{l=1}^N(y_l-Q_{\theta_i}(s_l, a_l))^2$
    \IF{$t$ mod $d$}
    \STATE // Update the actor with bias-shift;
    \STATE $b_{\mathrm{old}} \leftarrow b$
    \STATE Add $\ell_2$ regularization (Sec. \ref{Sec:regularization}):
     $ J \gets J+ \mathrm{Reg}(W, b)$
    \STATE Update $\phi$ by policy gradient:
     $\nabla_\phi J \gets \frac{1}{N}\sum\nabla_a Q_{\theta_1}|_{a=\pi_\phi}\nabla_\phi\pi_\phi+\nabla_\phi \mathrm{Reg}_{\phi}$
     
    \STATE Ensure bias magnitude:
    \textbf{if any entry of $b$ has magnitude less than $m$, revert it back to that of $b_{\mathrm{old}}$};
    %\IF{$|b|< m$}
    %\lin{in the above, it seems $|b|>m$, so why this happens?}
    %\STATE $b \leftarrow b_{old}$
    %\ENDIF
    \STATE Update target networks:\\
     $\qquad\theta_i' \leftarrow \tau \theta_i + (1 - \tau)\theta_i'$ and  $\phi' \leftarrow \tau\phi + (1 - \tau)\phi'$ for some learning rate $\tau>0$;
    %\lin{what is $\tau$?}
    \ENDIF
    %\IF{$steps > max$ or $done$}
    %\STATE Reset environment
    %\ENDIF
    \ENDFOR
\end{algorithmic}
\end{algorithm*}

\paragraph{Post-Training Adjustment}
To further ensure the actor output matches the linear controller, an additional step is made after the training.
The detailed algorithm is presented in Algorithm~\ref{Alg:optimize}.
In this algorithm, we fix \lin{complete this part ...}\textbf{EXPLAIN RELAXATION}
\begin{algorithm}[h]
   \caption{Optimize Actor Last Layer Parameters}
   \label{Alg:optimize}
\begin{algorithmic}[1]
    \IF{not relaxation}
    \STATE Solve Eq. \ref{Eq:opt_1} for last layer $\phi_{N, opt}$
    \STATE $\phi_N \leftarrow \phi_{opt}$
    \ELSE
    \WHILE{max(Real($\lambda$) of closed loop)$\ge0$ (Eq. \ref{Eq:closedloop_stable})}
    \STATE Solve Eq. \ref{Eq:opt_2} for last layer $\phi_{N, opt}$
    \STATE $\phi_N \leftarrow \phi_{opt}$
    \STATE Increment $\nu_{K}$
    \ENDWHILE
    \ENDIF
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[h]
   \caption{Bias Initialization}
   \label{Alg:bias_initialization}
\begin{algorithmic}[1]
    \STATE\textbf{Input: } linear region size: m$>$0;
    \STATE\textbf{Initialization:}
    \STATE Initialize biases: sample $b_l$ at layer $l$ by a random number from $[(-c_bm,-m)\cup (m, c_bm)]$  where $c_b>0$ is a parameter
    \IF{$l > 1$}
    \FOR{$\{b_l|W_l\hat{b}_m + b_l\}< m\}$ (Eq. \ref{Eq:ff_linear})}
    \WHILE{$W_l\hat{b}_m + b_l < m$}
    \STATE $b_l \leftarrow b_l + c\;\text{sign}(W_l\hat{b}_m)$ where $c$ is a parameter
    \ENDWHILE
    \ENDFOR
    \ENDIF
\end{algorithmic}
\end{algorithm}

%To capture the behavior of classical linear controllers, e.g., \emph{linear quadratic regulator} (LQR), a penalization term on the distance to the classical controller is added during training, and after training the last layer parameters are directly adjusted.
%To verify the effectiveness of our new approach, we analyze the performance of the resulting policy in both simulation and hardware. Our new policy achieves similar performance in the simulator as a non-modified neural networks. Examining the linear region of the system, we verify that our new policy effectively matches the prior-known LQR policy. We transfer our simulated policy to hardware. \lin{put performance here}. We believe our framework can \lin{write some hype words..}



% Dropping the activation function
If $b_{l,i} \ge m$, assuming that $|w_{l,i}^Tx_l| \le m$, the value passes through ReLU and returns itself, where $w_{l,i}$ denotes the vector notation of the rows of weight matrix $W_l$ transposed. If $b_{l,i} \le m$, the value saturates to zero after applying ReLU. The sign of $b$ determines how to appropriately mask $W_l$ and $b_{l,i}$ in such a way that ReLU can be dropped when calculating the output of the linear region:
\begin{equation}
       \sigma(w^T_{l,i}x_l+b_{l,i})= \begin{cases} 
        w^T_{l,i}x_l+b_{l,i}, & \text{if}\ b_{l,i} > 0\\ 
        0, & \text{if}\ b_{l,i} < 0\end{cases}    
\label{Eq:masking}
\end{equation}
% Simplification of linear region algebra
From Eq. \ref{Eq:masking} certain rows of $W$ and $b$ can be set to zero for the elements that ReLU saturates. In other words when $b_{l,i} < 0$, setting $w^T_{l,i}=0^T$ and $b_{l,i}=0$ achieves the same effect as applying ReLU. Let the subscript, $m$, denote appropriately masked parameters that are zeroed out to replicate the effects of ReLU. A two-layer network with ReLU activations helps illustrate how masking works:
\begin{equation}
\begin{split}
    \text{(1 Layer) }& y_{1,m} = W_{1,m} x+b_{1,m}\\
    \text{(2 Layers) }& y_{2,m} = (W_2W_{1,m})_m x+(W_2b_{1,m}+b_2)_m\\
\end{split}
\label{Eq:ff_linear_exp}
\end{equation}
Notice that for a two layer network $W_1$ and $b_1$ influence the cumulative masking. This means that the effective $b$ on the second layer is no longer just $b_2$; in fact, it is $W_2b_{1,m}+b_2$. The masking as a result for the second layer should be determined by the sign of $W_2b_{1,m}+b_2$. The effective gain on $x$ that needs to be masked is now $W_2W_{1,m}$ as opposed to $W_2$.

% Introduce LQR and Reinforcement Learning and make connection
%In this section and we briefly introduce reinforcement learning and linear quadratic regulator (LQR).
%Reinforcement learning and optimal control theory are closely intertwined, often trying to solve similar problems.
%Understanding how actor-critic style reinforcement learning algorithms relate to LQR will be crucial in understanding the fitting of the linear controller using our proposed netural network framework. 
%Note that this comparison is not limited to LQR but any stabilizing linear feedback controller. 
%For presentation simplicity, we consider mainly LQR throughout the paper.
%The main goal of both of these fields is to reduce cost and increase rewards which result in an optimal sequence of control inputs to achieving a task.

%Since RL does not require prior knowledge about the system to be controlled, it greatly reduces the difficulty of modeling complex systems. 
%However, in practice, it usually requires enormous examples/time to train in order to perform well.



%\lin{Give a brief intro of this algorithm hrere.}
%\textcolor{red}{For completeness, we give the detailed description of this algorithm in the appendix.}
%\lin{We need some intro of this algorithm. My suggestion would be add some text in the appendix about it.}
 %We adjust the initialization of biases in the actor and critic, and during training we added modest bias restrictions and crafted regularization terms when updating the actor parameters. An explicit reset of the environment was needed during training; otherwise, for certain environments it would flat line in performance and not improve at all. Our proposed techniques are not limited to TD3 but can be used with any actor-critic algorithm as long as the actor uses a feedforward function approximator. Please see Sec. \ref{Sec: Shifted-Bias Neural Network} for more details.
 
 %As we explained in the introduction, shifting the bias of a single ReLU is straightforward. 
%However, it is still not clear how to shift the bias of a multi-layer deep network so that resulting network has a linear region.
% Modifying the biases--overview
%Consider again the ReLU function of a layer,
%\[
%\sigma(Wx + b).
%\]
%Given a sufficiently large bias $b$, the ReLU function can be \emph{a prior} known to take on either $Wx+b$ or $0$ for a region of the input space. In the resulting linear region the activation operators can be disregarded with some slight modifications to $W$ and $b$. Moving the biases will alter where these linear regions lie, depicted in Fig. \ref{Fig:bias_constraints}. In this case, restricting the magnitude of the bias to be greater than $1$ ensures a linear output for $Wx \in (-1, 1)$.
%As such shifting the bias of a single ReLU is straightforward. 
%However, it is still not clear how to shift the bias of a multi-layer deep network so that resulting network has a linear region.





%Recall that our algorithm contains three phases: initialization, training, and post-training processing. 
%We will analyze each phase separately and combine the analysis in the end.

%In this section, we explain why our 
%``Bias-shifted'' refers to three aspects: initialization, training, and post-training processing. The initialization phase shifts the biases to be a desired magnitude corresponding to a desired region of the state space before training begins, constructing a linear region.During training earlier layers can compromise the linearity of the desired state space, so regularization terms are added in to counteract those effects. Post-training processing regularization terms are also added to the loss during training. This helps counter act the side effects when fitting to a controller post training.



% To initialize a linear region the cumulative effects of $W_n\hat{b}_m$ need to be added into the calculations. In practice we set $b$ in a sequential manner by uniformly sampling to until the total magnitude reaches the desired. As the combinations get more complex, we also can randomly sample $b$ and increment the value with the same sign as $W_n\hat{b}_m$ until the desired magnitude is met.
% In Algorithm~\ref{Alg:TD3training}, 
% any activation function can be used as long as it either contains a linear or approximately linear segment to establish a linear region. Throughout this paper ReLU will be used to demonstrate and formulate the optimization and examples here\textbf{ADD: Why ReLU and not sigmoid: Sigmoid experiences saturation during learning include cite}, but the generalized notation of $\sigma$ for activations will be kept throughout to indicate this can be used with other activation types. Each type of activation unit will require its own slight modifications to the constructions presented here.




% Modifying the biases--Feedforward layer

% Note that the critical difference between our algorithm and the original TD3 framework is the bias-shift step (Line~\textbf{Fill in ???}).
%the activation functions align in such a way that for a portion of the state space a feedforward network outputs a linear combination. Regularization terms on combinations of weights and biases are added to maintain the linear regions during training and nonlinear regions after training when weights are tuned to fit a linear controller. Despite the magnitude constraints and regularizers, Sec. \ref{Sec:Expressiveness and Loss Guidance} demonstrates how our method can greatly outperform the original implementation of TD3 and TD3 with DR on a pendulum.

% \section{Future Works}
% In the future we plan to implement this algorithm on an actual quadruped robot based off of \cite{kajita2003biped} controller. We also found a way to approximately fit the critics to the LQR solution. However, because it is only an approximation there are more obstacles that need to be dealt with before trying to implement this to avoid any sort of biasing of the critic when transferring to hardware.
